Deep Reactive Planning in Dynamic Environments

The main novelty of the proposed approach is that it allows a robot to learn an end-to-end policy which can adapt to changes in the environment during execution. While goal conditioning of policies has been studied in the RL literature, such approaches are not easily extended to cases where the robot's goal can change during execution. This is something that humans are naturally able to do. However, it is difficult for robots to learn such reflexes (i.e., to naturally respond to dynamic environments), especially when the goal location is not explicitly provided to the robot, and instead needs to be perceived through a vision sensor. In the current work, we present a method that can achieve such behavior by combining traditional kinematic planning, deep learning, and deep reinforcement learning in a synergistic fashion to generalize to arbitrary environments. We demonstrate the proposed approach for several reaching and pick-and-place tasks in simulation, as well as on a real system of a 6-DoF industrial manipulator. A video describing our work could be found \url{https://youtu.be/hE-Ew59GRPQ}.

==> exp_details.tex <==
% \section{Experimental Details}

% \subsection{Waypoints Generator}
% \paragraph{RRT* Settings}
% RRT*~\cite{karaman2011sampling} includes \textit{rewiring} process that reconnects randomly generated new node $x_{\rm new}$ and previously sampled vertex set $V$. That process includes a hyper-parameter $\gamma_{\rm RRT*}$ that defines the target nodes to which the newly generated node connect as.
% \begin{equation}
%     r({\rm card}(V)) = \min \{ \gamma_{\rm RRT*}(\log ( {\rm card}(V))/{\rm card}(V)) ^{1/d}, \eta \}.
% \end{equation}
% We used the hyperparameter as $\gamma_{\rm RRT*} = 0.1$.

% \paragraph{CNN Architecture}
% \Tref{tab:cnn_architecture} shows the architecture of the waypoints generator. It takes a depth image and generates $N^{waypoints}$ waypoints. The relative goal position/angles and current position/angles are concatenated near the top layer.
% \begin{table}[htbp]
%     \centering
%     \caption{Architecture of waypoints generator. The $n^{state}=3$ if it generates the tip position of the robot arm, or $n^{state}=6$ if joint angles.}
%     \begin{tabular}{cccc}
%         \toprule
%         Shape & Layer size & Stride & Type \\ \midrule
%         $128 \times 128 \times 1$ & - & - & Depth image \\
%         $64 \times 64 \times 32$ & $3 \times 3 \times 64$ & 2 & Convolution \\
%         $16 \times 16 \times 64$ & $3 \times 3 \times 128$ & 2 & Convolution \\
%         $4 \times 4 \times 128$ & $3 \times 3 \times 128$ & 2 & Convolution \\
%         $128$ & - & - & Global Average Pooling \\
%         $128 + 2 \times n^{state}$ & - & - & Concatenate image, relative goal location, and joint angles \\
%         $256$ & - & 256 & Fully Connected \\
%         $N^{waypoints} \times n^{state}$ & - & - & Output \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:cnn_architecture}
% \end{table}

% \subsection{Reinforcement Learning}


==> exp_sim2real.tex <==
% \section{sim2real: How to Bridge the Gap from Different Quality of Depth Camera?}

% \subsection{Hardware Setup}
% \subsubsection{Azure Kinect v.s. RealSense D435}
% First, we saw the difference between a real depth image (taken by the RealSense D435) and a simulated depth image from MuJoCo. \Fref{fig:real_sim_gap} shows the real image, simulated image, and the difference image.
% An obstacle (tissue box) is located in front of the robotic arm, whose size is $(W \times H \times D) = (0.122, 0.248, 0.114)$ [m].

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim_real_gap_1.png}
%     \includegraphics[width=0.8\textwidth]{fig/sim_real_gap_2.png}    \caption{Depth images obtained from a RealSense D435 sensor (left), the MuJoCo simulator (middle), and the difference between the real and simulated images (right). Blue region in the difference images indicates small difference between real and simulator depth images. Note that pixel values of the region where the distance is detected as more than $3$ meters is set to $0$ for easier comparison of the results. \konote{RealSense435 has already been replaced with Azure Kinect. I'll update this figure soon.}}
%     \label{fig:real_sim_gap}
% \end{figure}

% \subsubsection{Calibration of depth camera}

% \paragraph{Position of camera}
% The relative positions of the obstacle and camera is summarized in \Tref{tab:locations}.

% \begin{table}[htbp]
%     \centering
%     \caption{Relative location from the robotic arm.}
%     \begin{tabular}{l|cc} \toprule
%           & Obstacle [m] & Camera [m] \\ \midrule 
%          $X$ (directed out of the paper) & 0.30 & 1.56 \\
%          $Y$ (horizontal direction) & 0.00 & 0.09 \\
%          $Z$ (vertical direction) & 0.12 & 0.41 \\
%          \bottomrule
%     \end{tabular}
%     \label{tab:locations}
% \end{table}

% \paragraph{Pre-processing}
%     For the MuJoCo simulator, the raw pixel values $I^{raw}$ are first converted to real distance values. Referring to~\cite{dmcontrol}, the conversion can be computed as:
%     \begin{equation}
%     I^{dist}_{i,j} = p^{near} / (1 - I^{raw}_{i,j} \times (1 - p^{near} / p^{far})),
%     \end{equation}
%     where $I \in [0, 1]^{W \times H}$ is the depth image whose width and height is $W$ and $H$. The $p^{near}, p^{far}$ are camera parameters.
%     Then, clip only regions of interest distance $d_{min}, d_{max}$ as:
%     \begin{equation}
%     I^{fitted-dist}_{i,j} = \max(\min(I^{dist}_{i,k}, d_{max}), d_{min}),
%     \end{equation}
%     where we specifically use $(d_{min}, d_{max}) = (0.9, 2.0)$ [m] for our setting.
%     Finally, the pixel values are normalized so that the minimum value becomes $0$ and the maximum value becomes $1$.

% \paragraph{Other Tricks}
%     In order to get higher quality depth images, we cover the table with white papers. This significantly improves the quality of the image, because it prevents reflections of lights.
%     Also, we make bigger holes to make it stand out more in an image.

\input{exp_sim2real_cyclegan}
\input{exp_sim2real_waypoints}
\input{exp_sim2real_waypoints_no_obs}


==> exp_sim2real_waypoints.tex <==
% \subsection{Evaluate trained model: can it deal with the sim2real problem?}

% \paragraph{Create dataset}
% \Aref{alg:waypoints_dataset} shows the procedure to generate the waypoints dataset.
% The number of obstacles' locations and start-goal location is $N^{obs} = 5$, and $N^{random location} = 6 \times 6$ respectively.

% \begin{algorithm}
% 	\caption{The procedure to create the dataset}\label{alg:waypoints_dataset}
% 	\begin{algorithmic}[1]
%         \State Initialize $\tau$
%         \Comment{Buffer to store generated data}
%         \State \SIM{Generate RRT path $Z \in \{\bm{z}_1, ..., \bm{z}_T \}$ for different obstacle settings}
% 		\For{Given obstacles settings $\mathbb{O} \in {o_1, ..., o_N}$}
% 		\State \REAL{Load *.pkl file}
% 		\State \BOTH{Set obstacles to specified positions in both simulator and real system}
% 		\For{Given number of different random points}
%             \For{$\bm{z}_t \in Z$}
%                 \State \REAL{Set robot position or angle to $z_t$}
%                 \State \REAL{Take a depth image $I^{depth}$}
%                 \State $\tau \leftarrow \tau \cup \{I^{depth}\}$
%                 \Comment{Append the generated data to buffer}
%             \EndFor
%         \EndFor
%         \EndFor
% 	\end{algorithmic}
% \end{algorithm}

% \paragraph{Evaluate trained model}
% Candidate approaches to learn a robust model for waypoints generator.
% \begin{itemize}
%     \item Domain Randomization~\cite{tobin2017domain}
%     \item Domain Adaptation~\cite{ganin2014unsupervised}
% \end{itemize}

% \subsection{Azure Kinect}

% \subsubsection{Measure difference between real and simulation depth images}

% First, we saw the difference between real depth image (taken by Azure Kinect) and simulated depth image from MuJoCo. \Fref{fig:real_sim_gap} shows the real image, simulated image, and the difference image.
% An obstacle (tissue box) is located in front of the robotic arm, whose size is $(W \times H \times D) = (0.122, 0.248, 0.114)$ [m].
% The relative locations of the obstacle and camera is summarized in \Tref{tab:locations}.

% \begin{table}[htbp]
%     \centering
%     \caption{Relative location from the robotic arm.}
%     \begin{tabular}{l|cc} \toprule
%           & Obstacle [m] & Camera [m] \\ \midrule 
%          $X$ (directed out of the paper) & 0.30 & 1.56 \\
%          $Y$ (horizontal direction) & 0.00 & 0.09 \\
%          $Z$ (vertical direction) & 0.12 & 0.41 \\
%          \bottomrule
%     \end{tabular}
%     \label{tab:locations}
% \end{table}

% \subsubsection{Training with simulated depth images and evaluated on real images. (Baseline)} \label{exp:sim2real_baseline}
% In this experiment, the waypoints generator is trained on simulated depth images, and evaluated on real depth images.
% Both datasets consist of 585 steps (9 different goal location from the same start location).
% \Fref{fig:sim2real_baseline1} shows the loss curve.
% The test loss (real images) in 500 epochs is $7.28 \times 10^{-5}$, so the difference to the target position is $8.54 \times 10^{-2}$ [m]. 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_baseline1.png}
%     \caption{Training with simulated depth images and evaluated on real images.}
%     \label{fig:sim2real_baseline1}
% \end{figure}

% \subsubsection{Training with unrelated simulated depth images and evaluation on real images. (Baseline2))}
% This experiment uses 50,000 steps of simulated images for training, and evaluation is done both in simulation and on the real system, both of which are collected from the same trajectories as in the previous experiment in \sref{exp:sim2real_baseline}.
% Note that the distribution of robot movements between training and evaluation is different, so we would not expect the loss to become small, even in evaluation with simulated images.
% \Fref{fig:sim2real_baseline2} shows the loss curve. In the evaluation loss, the blue line is for simulated images, and the orange line is for images from the real system.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_baseline2.png}
%     \caption{Training with simulated depth images and evaluation on both simulated (blue line) and real system (orange line) images. Note that trajectories and locations of obstacles for training are sampled from different distribution from evaluation.}
%     \label{fig:sim2real_baseline2}
% \end{figure}

% \subsubsection{Training with unrelated simulated and real depth images and evaluation on real images. (Baseline3))}

% In this experiment, the waypoints generator is trained on simulated and real depth images, and evaluated on real depth images.
% The training dataset consists of about 5,000 steps (9 different start and goal locations from the same start location). The test dataset consists of 585 steps (9 different goal location from same start location) in \Fref{fig:sim2real_baseline3}

% The loss is calculated as $L_{categorical} - \alpha L_{binary}$

% Pre-experiment: MNIST

% The training dataset consists of about 60,000 images (half of the images are original, and the other half of the images are color-inverted images). The test dataset consists of 10,000 images  (half of the images are original, and the other half of the images are color-inverted images)  in \Fref{fig:sim2real_baseline3_mnist}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_baseline3_mnist.png}
%     \caption{Sample domain adaptation result for MNIST. (Original image:0, color inverted image:1)}
%     \label{fig:sim2real_baseline3_mnist}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_baseline3.png}
%     \caption{Sample domain adaptation result for robot arm. This NN outputs the next 5 steps pos and binary category (Sim:0, Real:1), orange: $\alpha=1e^{-6}$}
%     \label{fig:sim2real_baseline3}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_nn1.jpg}
%     \caption{Sample domain adaptation NN. This NN outputs the next 5 steps pos and binary category (Sim:0, Real:1)}
%     \label{fig:sim2real_nn1}
% \end{figure}

% \subsubsection{Training with unrelated simulated and real depth images and evaluation on real images. (Baseline4))}

% This experiments uses 50,000 steps of simulated images and about 5,000 steps (9 different start and goal locations from the same start location) of real images for training, and evaluation is done both in simulation and on the real system, both of which are collected from the same trajectories as in the previous experiment in \sref{exp:sim2real_baseline}. The result is shown in \Fref{fig:sim2real_baseline4}. Training binary loss is 0.9 and test binary loss is 0, and it means the NN predicts only 0 as a simulator image.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{fig/sim2real_baseline4.png}
%     \caption{Sample domain adaptation result for robot arm. This NN outputs next the 5 steps pos and binary category (Sim:0, Real:1) ($alpha=1e^{-6}$ gray: baseline4 setting, blue: baseline3 setting}
%     \label{fig:sim2real_baseline4}
% \end{figure}



==> exp_trajopt.tex <==
% \section{Peg Insertion in Cartesian Space}

% \subsection{Problem Setting}
% \subsubsection{MDP}
% \paragraph{State}
% The state of an agent is concatenation of current position $x_t$, relative goal position $x^{rel-goal}_t = x^{goal}_t - x_t$, and obstacle locations $x^{obs}_t$. Therefore, the state space will be $\mathcal{S} \in \mathbb{R}^{6 + 3 \times N^{obs}}$, where $N^{obs}$ is number of obstacles.
% If the agent takes the waypoints $\bm{z}_t$, then the state space will be $\mathcal{S} \in \mathbb{R}^{6 + 3 \times N^{obs} + 3 \times N^{waypoints}}$, where $N^{waypoints}$ is number of waypoints.
% \Tref{tab:state_space} summarizes the state space for each method.

% \begin{table}[htbp]
%     \centering
%     \small
%     \begin{tabular}{c|cccccc} \toprule
%         \multirow{2}{*}{Method}  & Position & Velocity & Relative goal & Waypoints & Depth image & VAE \\
%          & $x_t \in \mathbb{R}^{3}$ & $x_t \in \mathbb{R}^{3}$ & $x^\text{rel-goal}_t \in \mathbb{R}^{3}$ & $w_t \in \mathbb{R}^{3 \times 5}$ & $I^\text{depth}  \in \mathbb{R}^{64 \times 64 \times 1}$ & $z_t  \in \mathbb{R}^{64}$ \\
%          \midrule
%          \baseline    & O & O & O & - & - & - \\
%          \baselineimg & O & O & - & - & O & - \\
%          \baselinevae & O & O & - & - & - & O \\
%          \ours        & O & O & - & O & - & O \\
%          \ourswovae   & O & O & - & O & - & - \\
%          \bottomrule
%     \end{tabular}
%     \caption{State space for each method.}
%     \label{tab:state_space}
% \end{table}

% \paragraph{Action}
% The action of an agent is the relative next position $a^{rel}_t$. Since we suppose the underlying robot dynamics are unknown, and the robot can be operated by position control mode, which invariably reaches the specified position by using an internal controller, the dynamics of the robot will be $x_{t+1} = x_t + a^{rel}_t$.

% \paragraph{Initial settings}
% The start, goal, and obstacles' positions are randomly sampled from a position defined in \Tref{tab:randomization_area} when an episode starts. In order to imitate a pick-and-place task, the $Z$-axis area is set to smaller values than the height of obstacles.

% \begin{table}[htbp]
%     \centering
%     \caption{The randomization area from which start, goal, and obstacle positions are sampled. Note that the height ($Z$-axis value) of obstacles does not change due to a geometrical constraint.}
%     \begin{tabular}{cc|cc} \toprule
%          Type & Axis & Min. [m] & Max. [m] \\ \midrule 
%          \multirow{3}{*}{Obstacles}
%          & $X$ & 0.3 & 0.4 \\
%          & $Y$ & -0.3 & 0.3 \\
%          & $Z$ & - & - \\ \midrule
%         \multirow{3}{*}{Robot arm}
%          & $X$ & 0.2 & 0.4 \\
%          & $Y$ & -0.4 & 0.4 \\
%          & $Z$ & 0.05 & 0.3 \\ \midrule
%          \multirow{3}{*}{Start and Goal}
%          & $X$ & 0.2 & 0.4 \\
%          & $Y$ & -0.4 & 0.4 \\
%          & $Z$ & 0.05 & 0.05 \\
%          \bottomrule
%     \end{tabular}
%     \label{tab:randomization_area}
% \end{table}

% \paragraph{Termination conditions}
% The termination conditions of an episode are 1) the robot position is close enough to goal location ($\| x_t - x_t^{goal} \|_2^2 < 5e^{-3}$ [m] in our setting), 2) the number of steps of each episode is greater than $T = 150$.


% \subsection{Waypoints Generator}

% \begin{algorithm}
% 	\caption{The procedure to create the dataset}\label{alg:peg_dataset}
% 	\begin{algorithmic}[1]
%         \Require
%               \Statex Buffer size $N$.
% 	    \State Initialize a buffer $B$
% 	    \Repeat
%     	    \Repeat
%     	        \State Reset environment
%     	        \State Generate a path $\tau \in \{q_1, ..., q_T\}$ using Bi-directional RRT\*
%     	        \For{$j = 1$ to $T$}
%         		    \State Set robot position to $q_j$
%         		    \State Get a depth image $I^{depth}_j$ by the depth camera
%         		    \State $B \leftarrow B \cup \{(I^{wrist}_j, q_j), q_{j+1} \}$
%     		    \EndFor
%     	    \Until{Collect $N$ transitions}
%             \State Dump $B$ to a file
%             \State Train waypoints generator with $B$
%             \State Evaluate the success rate of waypoints generator while collecting failure cases $\tau^{failure}$
%         \Until{Evaluation success rate achieves more than 95 \%}
% 	\end{algorithmic}
% \end{algorithm}


% \subsubsection{Generate Dataset}

% \subsubsection{Evaluation}
% \paragraph{Evaluation Metrics}

% \begin{table}[htbp]
%     \centering
%     \caption{The randomization area from which start, goal, and obstacle positions in evaluation}
%     \begin{tabular}{cc|cc} \toprule
%          Type & Axis & Obstacle1 & Obsttacle2 \\ \midrule \multirow{2}{*}{Obstacle}
%          & $X$ & 0.3 & 0.3 \\
%          & $Y$ & -0.1 & 0.1 \\
%          & $Z$ & - & - \\
%          \bottomrule
%     \end{tabular}
%     \label{tab:randomization_area_eval}
% \end{table}
% Firstly, we evaluated the quality of generated waypoints.
% In order to evaluate the quality of generated waypoints, we compared the successes rate for the results when the start, goal and obstacle position are specified in Figure \ref{fig:eval_waypoint_generator}.
% Start and goal position is defined as relative position from the obstacle.
% The red and green points represent the start and goal position.
%  The robot arm reciprocated green and red positions, respectively, for each obstacle 2 position (shown in \Tref{tab:randomization_area_eval}. Totally, $2 \times 6 \times 6 \times 2 = 144$ trials are done in evaluation.

% \paragraph{TODO}
% \begin{itemize}
%     \item \sout{Visualize 5 waypoint in trajectory}
%     \item \sout{fix some bug (difference obstacle size between sim and real), Fix robot model for RV-4FRL-SH (Need to find STL files)}
%     \item \sout{make test Environment to evaluate in Fig.\ref{fig:eval_waypoint_generator}}
%     \item \sout{implement Bi-directional $RRT*$}
%     \item \sout{Confirm it can train in MCS environment}
%     \item \sout{decrease the distance from next steps}
%     \item \sout{Evaluate average success rate in  \Tref{tab:xyz_waypoints_accuracy}}
% \end{itemize}
% \paragraph{Problems}
% \begin{itemize}
%     \item Train loss and test loss is almost the same (2e-4)
%     \item Robot arm can reach goal position from start position in a straight line, but the arm collide with obstacle.
% \end{itemize}

% \paragraph{Now trying}
% \begin{itemize}
%     \item
% \end{itemize}


% \begin{figure*}[htbp]
%     \begin{center}
%         \includegraphics[width=10cm]{fig/wp_evaluate.png}
%     \end{center}
%     \caption{the method to evaluate the waypoint generator in setting obstacle1 shown in \Tref{tab:randomization_area_eval}}
%     \label{fig:eval_waypoint_generator}
% \end{figure*}


% \begin{table}[htbp]
%     \centering
%     \caption{Average success rate with obstacles over 144 random start, goal, obstacles conditions.}
%     \begin{tabular}{c|c|ccc} \toprule
%         \multirow{2}{*}{\# obstacles} & \multirow{2}{*}{-} & \multicolumn{3}{c}{\# training data} \\
%         & & $10000$ & $25000$ & $50000$\\ \midrule 
%         1 & \# collision & 0.438 & 0.528 & 0.715\\
%         3 & \# collision &  &  &\\
%         5 & \# collision &  &  &\\
%         \bottomrule
%     \end{tabular}
%     \label{tab:xyz_waypoints_accuracy}
% \end{table}

% \subsection{Reinforcement Learning for Trajectory Optimization}



% \subsection{E2E experiments on simpler settings}
% \Fref{fig:preliminary_exp} shows the simpler setting to validate the whole system: starting from trajectory optimization and finish with connector insertion. We prepared three settings for that and report results in the following sections.
% The randomization area is specified in \Tref{tab:randomization_area_preliminary_exp}. Note that if an object is \textbf{fixed}, then the position becomes the average of the minimum and maximum positions. For example, if the start position of the robot arm is fixed, then the start position will be $(X,Y,Z)=(0.3, -0.3, 0.05)$.
% longer

% \clearpage
% \subsubsection{RL performance}
% \paragraph{Performance of the waypoints generator}
% \Fref{fig:rl_results_app} shows the results. It shows that \ours performs best in terms of both sample efficiency and final performance.
% Since \baseline and \ourswovae do not have spatial information about the environment, they cannot avoid collision with obstacles during training.

% \begin{figure*}[t]
% 	\begin{minipage}[]{0.5\linewidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{fig/results_average_return_3.0M_steps.png}
% 		\subcaption{Average return (higher is better)}\label{fig:results_return}
% 	\end{minipage}
% 	\begin{minipage}[]{0.5\linewidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{fig/results_average_steps_to_reach_goal_3.0M_steps.png}
% 		\subcaption{Average number of steps to reach goal (lower is better)}\label{fig:results_steps}
% 	\end{minipage}
% 	\begin{minipage}[]{0.5\linewidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{fig/results_average_goal_reach_rate_3.0M_steps.png}
% 		\subcaption{Average goal reach rate (higher is better)}\label{fig:results_goal_rate}
% 	\end{minipage}
% 	\begin{minipage}[]{0.5\linewidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{fig/results_average_times_to_collide_3.0M_steps.png}
% 		\subcaption{Average number of collision with obstacles (lower is better)}\label{fig:results_n_collision}
% 	\end{minipage}
% 	\caption{Training curves on each training type. The solid lines represent average returns over five instances with different random seeds. The shaded region represents the standard deviation of the five instances. Our approach outperforms the baseline in both sample efficiency and final performance.}
% 	\label{fig:rl_results_app}
% \end{figure*}

% \paragraph{Generalization performance}

% \begin{table*}[tbp]
% 	\caption{Performance on generalization task in simulation. The results are averaged over $200$ episodes with random agent, goal, obstacles locations.
% 	         The bold number indicates the best results among three different methods. In the ``Ours Fine-tuned'', we used the fine-tuned waypoints generator to improve the quality of waypoints. Note we do not retrain the RL agent.}
% 	\label{table:goal_param_success_rate}
% 	\begin{center}
% 	    \small
%             \begin{tabular}{ccccc} \toprule
%             \multirow{2}{*}{Environment}
%             & \multicolumn{4}{c}{Goal reach rate}\\
%                   \cmidrule{2-5}
%             & Baseline Image & Baseline VAE  & Ours & Ours VAE \\ \midrule
%             \textit{One obs} & 0.21 & 0.49 & \textbf{0.95} & 0.78 \\
%             \textit{Two obs} & 0.16 & 0.34 & \textbf{0.92} & 0.69 \\
%             \textit{Three obs} & 0.15 & 0.34 & \textbf{0.89} & 0.72 \\
% 		    \bottomrule
% 	\end{tabular}
% 	\end{center}
% \end{table*}

